CARLA Drone: Monocular 3D Object Detection from a Different Perspective

Existing techniques for monocular 3D detection have a serious restriction. They tend to perform well only on a limited set of benchmarks, faring well either on ego-centric car views or on traffic camera views, but rarely on both. To encourage progress, this work advocates for an extended evaluation of 3D detection frameworks across different camera perspectives. We make two key contributions. First, we introduce the CARLA Drone dataset, CDrone. Simulating drone views, it substantially expands the diversity of camera perspectives in existing benchmarks. Despite its synthetic nature, CDrone represents a real-world challenge. To show this, we confirm that previous techniques struggle to perform well both on CDrone and a real-world 3D drone dataset. Second, we develop an effective data augmentation pipeline called GroundMix. Its distinguishing element is the use of the ground for creating 3D-consistent augmentation of a training image. GroundMix significantly boosts the detection accuracy of a lightweight one-stage detector. In our expanded evaluation, we achieve the average precision on par with or substantially higher than the previous state of the art across all tested datasets.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> supp_exp_ablation.tex <==
\begin{table}[t]
    \scriptsize
    \caption{\textbf{Ablation study of soft patch pasting.} The evaluation uses a subset of Rope3D \cite{main-Rope3D}. We study the effect of hard mining and compare to an alternative pasting strategy, Mix-Teaching \cite{main-mix-teaching}. We report $AP_{3D|R40}$ with $IoU = 0.5$.}
    \centering
    \begin{tabularx}{\linewidth}{
        @{}X @{\hspace{1em}}
        S[table-format=2.1]@{\hspace{1em}}
        S[table-format=2.1]
        }
      \toprule
      Method & Car & {Big Vehicle} \\
      \midrule
      \ourmethod & 44.1 & 28.4 \\
      w/o hard mining & 42.8 & 26.9 \\
      w/ Mix-Teaching \cite{main-mix-teaching} & 42.6 & 27.0 \\
      \bottomrule
      \end{tabularx}

    \label{tab:supp_ablation}
\end{table}

==> supp_exp_qualit.tex <==
\begin{figure}[t]
%\setlength\extrarowheight{2pt} % for a slightly more open "look"
\centering
\begin{tabular}{c c c}

\includegraphics[height=66pt]{supp_exp_qualit_waymo_monocon.png} &
\includegraphics[height=66pt]{supp_exp_qualit_rope3d_monocon.jpg} &
\includegraphics[height=66pt]{supp_exp_qualit_cdrone_monocon.jpg} \\

\includegraphics[height=66pt]{supp_exp_qualit_waymo_ours.png} &
\includegraphics[height=66pt]{supp_exp_qualit_rope3d_ours.jpg}& 
\includegraphics[height=66pt]{supp_exp_qualit_cdrone_ours.jpg} \\

\end{tabular}
\caption{\textbf{Qualitative Results. } We compare our baseline MonoCon \cite{main-monocon} (first row) with \ourmethod (second row). For MonoCon \cite{main-monocon} we extend the single angle into a full 3D rotation using the provided ground normal. The column indicates the dataset: Waymo \cite{main-waymo} (first column), Rope3D \cite{main-Rope3D} (second column), CDrone (third column).}
\label{fig:supp_qual_results}
\end{figure}

==> supp_exp_qualit_real_drone.tex <==

\begin{figure}[t]
%\setlength\extrarowheight{2pt} % for a slightly more open "look"
\centering
\begin{tabular}{c c c}

\includegraphics[height=115pt]{supp_exp_qualit_real_1_monocon.png} &
\includegraphics[height=115pt]{supp_exp_qualit_real_2_monocon.png} &
\includegraphics[height=115pt]{supp_exp_qualit_real_3_monocon.png}
\\

\includegraphics[height=115pt]{supp_exp_qualit_real_1_ours.png}& 
\includegraphics[height=115pt]{supp_exp_qualit_real_2_ours.png} &
\includegraphics[height=115pt]{supp_exp_qualit_real_3_ours.png}
\\

\end{tabular}
\caption{\textbf{Qualitative Results. } We compare our baseline MonoCon \cite{main-monocon} (first row) with \ourmethod (second row) on the in-house real drone dataset. Our approach predicts more accurate 3D box rotation and dimensions while leading to fewer false positives.}
\label{fig:qual_results_real_drone}
\end{figure}

==> supp_exp_waymo_full.tex <==
\begin{table*}[t]
    \caption{\textbf{3D detection accuracy on Waymo (val).} We use the data splits proposed by Reading \etal~\cite{main-waymo} for training and validation, and report the accuracy for the vehicle class across various distance thresholds. \ourmethod improves over the baseline and can operate across all camera views in our benchmark: the car view (C), the traffic camera view (T) and the drone view (D).}
    %$^*$DEVIANT\cite{main-DEVIANT} uses GUPNet \cite{main-GUPNet}, which is designed for car view \cite{main-MONOUNI}. 
    \setlength \scriptsize
    \centering
    \medskip
    %\resizebox{1.0\textwidth}{!}
    \begin{tabularx}{\linewidth}{
        @{}c  c  X  ccc @{\hspace{1em}}
        *{2}{S[table-format=2.2]@{\hspace{0.5em}}}
        S[table-format=2.2]@{\hspace{0.5em}}
        S[table-format=1.2]@{\hspace{1em}}
        *{2}{S[table-format=2.2]@{\hspace{0.5em}}} 
        *{1}{S[table-format=1.2]@{\hspace{0.5em}}} 
        S[table-format=1.2]}
        
      \toprule
      \multirow{2}{*}{IoU} & \multirow{2}{*}{Level} & \multirow{2}{*}{Method} & \multirow{2}{*}{C} & \multirow{2}{*}{T} & \multirow{2}{*}{D} & \multicolumn{4}{c}{$AP_{3D} \uparrow$} & \multicolumn{4}{c}{$APH_{3D} \uparrow$} \\
      \cmidrule(lr){7-10} \cmidrule(lr){11-14}
      & & & & & & {All} & {0-30} & {30-50} & {50-$\infty$} & {All} & {0-30} & {30-50} & {50-$\infty$} \\ \midrule
      
      \multirow{2}{*}{0.7} & \multirow{2}{*}{1} & MonoCon \cite{main-monocon,main-choi2023depthdiscriminative} & \cmark & \cmark &  & 2.30 & 6.66 & 0.67 & 0.02 & 2.29 & 6.62 & 0.66 & 0.02 \\
      & & \ourmethod (Ours) & \cmark & \cmark & \cmark & \textbf{3.10} & \textbf{8.94} & \textbf{1.17} & \textbf{0.06} & \textbf{3.08} & \textbf{8.88} & \textbf{1.16} & \textbf{0.06} \\ \midrule

      \multirow{2}{*}{0.7} & \multirow{2}{*}{2} & MonoCon \cite{main-monocon,main-choi2023depthdiscriminative}  & \cmark & \cmark &  & 2.16 & 6.64 & 0.64 & 0.02 & 2.15 & 6.59 & 0.64 & 0.02 \\
       & & \ourmethod (Ours) & \cmark & \cmark & \cmark & \textbf{2.73} & \textbf{8.81} & \textbf{1.06} & \textbf{0.04} & \textbf{2.71} & \textbf{8.75} & \textbf{1.05} & \textbf{0.04} \\  \midrule

      \multirow{2}{*}{0.5} & \multirow{2}{*}{1} & MonoCon \cite{main-monocon,main-choi2023depthdiscriminative}  & \cmark & \cmark &  &  10.07 & 27.47 & 3.84 & 0.17 & 9.99 & 27.26 & 3.81 & 0.16\\
       & & \ourmethod (Ours) & \cmark & \cmark & \cmark &  \textbf{11.89} & \textbf{30.87} & \textbf{6.07} & \textbf{0.35} & \textbf{11.79} & \textbf{30.62} & \textbf{6.03} & \textbf{0.34} \\ \midrule

      \multirow{2}{*}{0.5} & \multirow{2}{*}{2} & MonoCon \cite{main-monocon,main-choi2023depthdiscriminative}  & \cmark & \cmark &  &  9.44 & 27.37 & 3.71 & 0.14 & 9.37 & 27.17 & 3.68 & 0.14 \\
       & & \ourmethod (Ours) & \cmark & \cmark & \cmark &  \textbf{10.50} & \textbf{30.48} & \textbf{5.52} & \textbf{0.27} & \textbf{10.42} & \textbf{30.24} & \textbf{5.48} & \textbf{0.27} \\
      
      \bottomrule
    \end{tabularx}
    \vspace{0.5em}

    \label{tab:waymo_full}
\end{table*}

==> supp_exp_waymo_lvl1.tex <==
\begin{table*}[t]
    \scriptsize
    \caption{\textbf{3D detection accuracy on Waymo (val).} We use the data splits proposed by Reading \etal~\cite{main-waymo} for training and validation, and report the accuracy for the vehicle class on Level 1 \cite{main-waymo} (the degree of difficulty). \ourmethod improves over the baseline while being applicable across all camera views in our benchmark: the car view (C), the traffic camera view (T) and the drone view (D). The full evaluation, provided in the \suppmat due to space constraints, is consistent with this conclusion.}
    %$^*$DEVIANT\cite{DEVIANT} uses GUPNet \cite{GUPNet}, which is designed for car view \cite{MONOUNI}. 
    %\setlength \scriptsize
    \centering
    \medskip
    %\resizebox{1.0\textwidth}{!}
    \begin{tabularx}{\linewidth}{
        @{}X c@{\hspace{0.5em}}c@{\hspace{0.5em}}c@{\hspace{0.8em}}
        *{2}{S[table-format=2.2]@{\hspace{1em}}}
        S[table-format=2.2]@{\hspace{0.8em}}
        S[table-format=1.2]@{\hspace{1em}}
        *{2}{S[table-format=2.2]@{\hspace{1em}}}
        S[table-format=1.2]@{\hspace{0.8em}}
        S[table-format=1.2]}
        
    %\begin{tabular}{l | c | c | c | c c c c | c c c c}
      %\Xhline{1pt}
      \toprule
      \multirow{2}{*}{Method} & \multirow{2}{*}{C} & \multirow{2}{*}{T} & \multirow{2}{*}{D} & \multicolumn{4}{c}{$AP_{3D} \uparrow$ $(\text{IoU} = 0.5)$} & \multicolumn{4}{c}{$AP_{3D} \uparrow$ ($\text{IoU} = 0.7$)} \\
      \cmidrule(lr){5-8} \cmidrule(lr){9-12}
      & & & & {All} & {0-30} & {30-50} & {50-$\infty$} & {All} & {0-30} & {30-50} & {50-$\infty$} \\ 
      %\hline
      %\Xhline{1}
      \midrule
      \textbf{With extra data} \\
      Stereoscopic \cite{stereoscopic} & \cmark & & & 7.18 & 22.85 & 5.40 & 1.52 & 1.72 & 6.98 & 1.52 & 0.48 \\
      PatchNet~\cite{PatchNet,PCT} & \cmark & \cmark &  & 2.92 & 10.03 & 1.09 & 0.23 & 0.39 & 1.67 & 0.13 & 0.03  \\
      PCT~\cite{PCT} & \cmark & \cmark & & 4.20 & 14.70 & 1.78 & 0.39 & 0.89 & 3.18 & 0.27 & 0.07 \\
      CaDDN \cite{main-CaDDN} & \cmark & \cmark & &  17.54 & 45.00 & 9.24 & 0.64 & 4.99 & 14.43 & 1.45 & 0.10 \\
      DID-M3D \cite{DID-M3D}  & \cmark & \cmark & & 20.66 & 40.92 & 15.63 & 5.35 & {---} & {---} & {---} & {---}\\
      TempM3D \cite{tempm3d} & \cmark & \cmark & &  23.95 & 45.46 & 19.50 & 6.31 & {---} & {---} & {---} & {---}\\
      MonoNeRD \cite{mononerd} & \cmark & \cmark & & 31.18 & 61.11 & 26.08 & 6.60 & 10.66 & 27.84 & 5.40 & 0.72 \\
      OccupancyM3D \cite{occupancyM3D} & \cmark & \cmark & & 28.99 & 61.24 & 23.25 & 3.65 & 10.61 & 29.18 & 4.49 & 0.41 \\

      \textbf{Without extra data} \\ 
      M3D-RPN~\cite{main-M3D-RPN,main-CaDDN} & \cmark & & & 3.79 & 11.14 & 2.16 & 0.26 & 0.35 & 1.12 & 0.18 & 0.02 \\      

      GUPNet~\cite{main-GUPNet,main-DEVIANT} & \cmark & & & 10.02 & 24.78 & 4.84 & 0.22 & 2.28 & 6.15 & 0.81 & 0.03 \\  
      DEVIANT$^*$ ~\cite{main-DEVIANT} & \cmark & && 10.98 & 26.85 & 5.13 & 0.18  & 2.69 & 6.95 & 0.99 & 0.02  \\
      MonoRCNN++ \cite{main-MonoRCNN++} & \cmark & & & 11.37 & 27.95 & 4.07 & 0.42 & 4.28 & 9.84 & 0.91 & 0.09 \\
      MonoJSG \cite{main-MonoJSG} & \cmark & \cmark & & 5.65 & 20.86 & 3.91 & 0.97 & 0.97 & 4.65 & 0.55 & 0.10 \\
      MonoLSS \cite{main-monolss} & \cmark & \cmark & & 13.49 & 33.64 & 6.45 & 1.29 & 3.71 & 9.82 & 1.14 & 0.16 \\
      MonoUNI \cite{main-MONOUNI} & \cmark & \cmark & & 10.98 & 26.63 & 4.04 & 0.57 & 3.20 & 8.61 & 0.87 & 0.13 \\
      SSD-MonoDETR \cite{ssd-monodetr} & \cmark & \cmark & & 11.83 & 27.69 & 5.33 & 0.85 & 4.54 & 9.93& 1.18 & 0.15 \\
      MonoXiver-GUPNet \cite{main-monoxiver} & \cmark & \cmark & & 11.47 & {---} & {---} & {---} & {---} & {---} & {---} & {---} \\      
      MonoXiver-DEVIANT \cite{main-monoxiver} & \cmark & \cmark & & 11.88 & {---} & {---} & {---} & {---} & {---} & {---} & {---} \\
      MonoCon \cite{main-monocon} + DDML \cite{main-choi2023depthdiscriminative} & \cmark & \cmark & & 10.14 & 28.51 & 3.99 & 0.17 & 2.50 & 7.62 & 0.72 & 0.02 \\ \midrule
      MonoCon {\scriptsize (Baseline)} \cite{main-monocon,main-choi2023depthdiscriminative} & \cmark & \cmark & & 10.07 & 27.47 & 3.84 & 0.17 & 2.30 & 6.66 & 0.67 & 0.02 \\ 
      
      
      
      \ourmethod~{\scriptsize (Ours)} & \cmark & \cmark & \cmark & 11.89 & 30.87 & 6.07 & 0.35  & 3.10 & 8.94 & 1.17 & 0.06\\
      \bottomrule

      %\Xhline{1pt}

    \end{tabularx}
    \vspace{0.5em}

    \label{tab:waymo_lvl1}
\end{table*}

==> supp_groundmix_imgs.tex <==
\begin{figure}[t]
%\setlength\extrarowheight{2pt} % for a slightly more open "look"
\centering
%\begin{tabular}{l r}
\minipage{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/supp_groundmix1.png}
\endminipage \,
\minipage{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/supp_groundmix2.pdf}
\endminipage \,
\minipage{0.13\textwidth}
\includesvg[width=\textwidth]{figures/supp_groundmix3.svg}
\endminipage \,
\minipage{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/supp_groundmix4.png}
\endminipage \,
\minipage{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/supp_groundmix5.png}
\endminipage\hfill
%\end{tabular}
\caption{\textbf{Soft pasting in comparison with pasting of Mix-Teaching \cite{main-mix-teaching}. } \textbf{Image 1:} The patch to be pasted. \textbf{Image 2:} Sampling of the mask ($a_1, a_2 \in [0, 10\%\cdot A]$, $b_1, b_2 \in [0, 20\%\cdot B]$) \textbf{Image 3:} The corresponding mask, where black denotes 0\% opacity and white denotes 100\% opacity. \textbf{Image 4:} Result after pasting the object softly with the mask of image 3. \textbf{Image 5:} Pasting as done in Mix-Teaching \cite{main-mix-teaching}. In contrast to Mix-Teaching \cite{main-mix-teaching}, our approach does not provide the network hints about the 2D bounding box .} 
\label{tab:patch_pasting}
\end{figure}

==> supp_method_mono3d_methods.tex <==

%\begin{wraptable}[18]{r}{1.0\textwidth}
\begin{table*}[t]
    \caption{\textbf{Monocular 3D detection methods in comparison. } We show, whether car view (C), traffic camera view (T) and drone view (D) fulfill the assumptions of the corresponding methods. }
    %\centering
    \scriptsize
    \begin{tabularx}{\linewidth}{
        @{}X c@{\hspace{0.7em}}
             c@{\hspace{0.7em}}
             c@{\hspace{2em}}
             l}
        
      \toprule
      Method & C & T & D & Architecture \\ \midrule
      
      MonoRCNN++ \cite{main-MonoRCNN++} & \cmark & & & Two-Stage \\
      Cube R-CNN \cite{main-omni3d} & \cmark & \cmark & \cmark & Two-Stage \\ \midrule

      GUPNet \cite{main-GUPNet} & \cmark & & & One-Stage \\
      MonoFlex \cite{main-Monoflex} & \cmark & & & One-Stage \\
      DEVIANT \cite{main-DEVIANT} & \cmark & & & One-Stage \\
      MonoDDE \cite{main-MonoDDE} & \cmark & &  & One-Stage \\
      M3D-RPN \cite{main-M3D-RPN} & \cmark & & & One-Stage \\
      MonoUNI \cite{main-MONOUNI} & \cmark & \cmark & & One-stage \\
      MonoGAE \cite{main-MonoGAE} & & \cmark & & One-Stage \\ \midrule
      BEVFormer \cite{main-BEVFormer} & \cmark & \cmark & & BEV \\
      BEVDepth \cite{main-bevdepth} & \cmark & \cmark & & BEV \\
      BEVHeight \cite{main-BEVHeight} & & \cmark & & BEV \\ 
      \midrule
      This work & \cmark & \cmark & \cmark & One-Stage \\
    \bottomrule
    \end{tabularx}
    \label{tab:methods}
\end{table*}
%\end{wraptable}
